Virasoro and Kac-Moody algebra in generic tensor network representations of 2d critical lattice partition functions

In this paper, we propose a general implementation of the Virasoro generators and Kac-Moody currents in generic tensor network representations of 2-dimensional critical lattice models. Our proposal works even when a quantum Hamiltonian of the lattice model is not available, which is the case in many numerical computations involving numerical blockings. We tested our proposal on the 2d Ising model, and also the dimer model, which works to high accuracy even with a fairly small system size. Our method makes use of eigenstates of a small cylinder to generate descendant states in a larger cylinder, suggesting some intricate algebraic relations between lattice of different sizes.

==> to be submitted to arxiv/appendices.tex <==
\subsection{Cylinder eigenstates and CFT spectra}

The partition function of a torus CFT can be written as:
\begin{align}
     Z_{\text{CFT}}
  &= \Tr \Bigl[
       \exp \bigl( -2\pi\Im\tau \cdot H_{\text{CFT}} \bigr)
       \exp \bigl(  2\pi\Re\tau \cdot P \bigr)
     \Bigr] \notag \\
  &= \Tr \Bigl[
       \exp \Bigl( -2\pi\Im\tau \Bigl( L_0 + \bar{L}_0 - \frac{c}{12} \Bigr) \Bigr)
       \exp \Bigl(  2\pi\Re\tau \bigl( L_0 - \bar{L}_0 \bigr) \Bigr)
     \Bigr].
\end{align}
Here, operators $H_{\text{CFT}}$ and $P$ denote the Hamiltonian and the total momentum operators that generate translations along the time and space directions, while $c$ is the central charge. $\tau$ is a complex modular parameter that parametrizes the geometry of the torus.

For a local field $\phi_\alpha$ with conformal dimension $(h_\alpha,\bar{h}_\alpha)$, from Virasogo algebra we know that
\begin{align}
     Z_{\text{CFT}}
  &= \sum_\alpha \exp \Bigl[
       - 2\pi    \Im\tau \Bigl( h_0 + \bar{h}_0 - \frac{c}{12} \Bigr)
       + 2\pi\iu \Re\tau \bigl( h_0 - \bar{h}_0 \bigr)
     \Bigr] \notag \\
  &= \sum_\alpha \exp \Bigl[
       - 2\pi    \Im\tau \Bigl(\Delta_\alpha - \frac{c}{12} \Bigr)
       + 2\pi\iu \Re\tau \cdot s_\alpha
     \Bigr],
\end{align}
where $\Delta_\alpha=h_0+\bar{h}_0$ and $s_\alpha=h_0-\bar{h}_0$ are the scaling dimension and conformal spin of $\phi_\alpha$ respectively.

In the continuum limit, a critical classical lattice model with periodic boundary conditions can be described by the torus CFT, with modular parameter $\tau=\iu m/N$. The partition function is then
\begin{equation}
  Z = \sum_\alpha \exp \Bigl[
      - 2\pi \frac{m}{N} \Bigl(\Delta_\alpha - \frac{c}{12} \Bigr)
      + mNf + \mathcal{O} \Bigl( \frac{m}{N^\gamma} \Bigr)
    \Bigr],
\end{equation}
where $f$ is the free energy per each site at the thermodynamic limit, and $\mathcal{O}(m/N^\gamma)$ is the finite-size corrections. If the partition function can be written as $Z=\Tr M^m$ where $M$ is the transfer matrix, the eigenvalues of $M$ are then
\begin{equation}
  \lambda_\alpha = \exp \Bigl[
    - \frac{2\pi}{N} \Bigl( \Delta_\alpha-\frac{c}{12} \Bigr)
    + Nf + \mathcal{O} \Bigl( \frac{1}{N^\gamma} \Bigr)
  \Bigr].
\end{equation}
The conformal spin can be calculated by introducing the translation operator $\exp(2\pi\iu P/N)$, whose eigenvalues are $\exp(2\pi\iu s_\alpha/N)$. For a translationally invariant model, $\exp(2\pi\iu P/N)$ commutes with the transfer matrix $M$, so they can be diagonalized simultaneously to produce a set of eigenvectors with eigenvalues $ \{ \lambda, P_\alpha \}$. One way of estimate the scaling dimension $\Delta_\alpha$ is to fix the identity state $\ket{\phi_I}$ and state $\ket{\phi_T}$ corresponding to energy momentum tensor to have $\Delta_I=0$ and $\Delta_T=2$ so that
\begin{equation}
\Delta_\alpha = \frac{2}{\log \lambda_T - \log \lambda_I} \left( \log \lambda_\alpha - \log \lambda_I \right) .
\end{equation}
Conformal spin is obtained from the eigenvalues of the lattice translation operator $P$ as
\begin{equation}
s_\alpha = \frac{N}{2\pi} P_\alpha .
\end{equation}

\subsection{Numerical details for the Ising model}

\definecolor{blue1}{RGB}{10,120,180}
\definecolor{blue2}{RGB}{107,175,215}
\newcommand{\good}{\color{blue1}\bfseries}
\newcommand{\bad}{\color{blue2}}

\input{isingmel}
\clearpage

\subsection{Numerical details for the dimer model}

\input{dimermel}

==> to be submitted to arxiv/dimermel.tex <==
Similar to the Virasoro algebra case, we start by combining dimer model tensor $B^{(0)}$ into $2\times2$ square block to get a new tensor $B=B^{(1)}$ of bond dimension $\chi=4$ and then extract the approximate local current tensor $J$ operator and its holomorphic part $\bar{J}$ from a smaller cylinder of $N=4$ copies of coarse-grained tensor $B$.  $J$ and $\bar{J}$ are then used to construct Kac--Moody generators $J_n$ and $J_{-n}$ on a larger $N=8$ cylinder.

We verify the actions of the lattice Kac--Moody generators by examining the matrix elements $\mel{\phi_\alpha}{J_n}{\phi_\beta}$ and $\mel{\phi_\alpha}{\bar{J}_{n}}{\phi_\beta}$ with $n=-1, -2$ using the low energy eigenstates from a cylinder of $N=8$ sites of $B$. Numerical results of the matrix elements are provided in Table~\ref{tab:dimer_jm1}--\ref{tab:dimer_jm_2_jbarm2} and their behaviors in the low energy subspace are illustrated in Fig.~\ref{fig:j1j2}. The matrix elements between states and their correct Kac--Moody descendant states are highlighted in bold blue in the tables and illustrated correspondingly by solid black arrows in the figures. The erroneous matrix elements are marked in pale blue in the tables and illustrated by dashed gray arrows in the figures.

\begin{figure}[htb]
  \centering
  \subfloat[$J_{-1}$]{
    \includegraphics[width=0.32\textwidth]{dimer_jm1.pdf}
    \label{fig:dimer_jm1}}
  \qquad
  \subfloat[$\bar{J}_{-1}$]{
    \includegraphics[width=0.32\textwidth]{dimer_jbarm1.pdf}
    \label{fig:dimer_jbarm1}}
  \\
  \subfloat[$J_{-2}$]{
    \includegraphics[width=0.32\textwidth]{dimer_jm2.pdf}
    \label{fig:dimer_jm2}}
  \qquad
  \subfloat[$\bar{J}_{-2}$]{
    \includegraphics[width=0.32\textwidth]{dimer_jbarm2.pdf}
    \label{fig:dimer_jbarm2}}
  \caption{Actions of lattice Kac--Moody generators $J_{-1, -2}$ and $\bar{J}_{-1, -2}$ in the low energy subspace of transfer matrix consisting of a row of $N=8$ copies of $B$ with bond dimension $\chi=4$. Corresponding matrix elements are listed in Table~\ref{tab:dimer_jm1}--\ref{tab:dimer_jm_2_jbarm2}.}
  \label{fig:j1j2}
\end{figure}

\begin{table}[htb]
  \centering\small
  \def\M#1{$\mel{\phi_\alpha}{J_{-1}}{#1}$}
  \begin{tabular}{*{10}{c}}
    \toprule
    $\ket{\phi_\alpha}$ & $\Delta_\alpha$ & $(s_\alpha, \Delta^{\text{exact}}_\alpha)$ & \M{1} & \M{2} & \M{4} & \M{8} & \M{9} & \M{10} & \M{14} \\
    \midrule
    1  & 0.000 & (0, 0)      & 3.266e-16       & 9.883e-17       & 6.044e-11       & \bad 2.757e-01  & 9.948e-12       & 2.562e-15       & 2.663e-17 \\
    2  & 0.238 & (0, 1/4)    & 1.064e-16       & 7.638e-16       & 4.130e-16       & 9.487e-15       & 5.270e-16       & \bad 3.124e-01  & 5.666e-11 \\
    3  & 0.238 & (0, 1/4)    & 4.070e-16       & 9.022e-16       & 5.978e-16       & 5.873e-15       & 6.256e-16       & \bad 1.838e-01  & 3.055e-11 \\
    4  & 0.959 & (0, 1)      & 6.138e-11       & 2.088e-15       & 2.491e-11       & \bad 2.632e-01  & 9.498e-12       & 1.912e-15       & 3.097e-17 \\
    5  & 0.959 & (0, 1)      & 1.089e-11       & 5.677e-15       & 1.069e-10       & \bad 4.899e-01  & 1.768e-11       & 5.352e-16       & 7.399e-17 \\
    6  & 0.959 & (0, 1)      & 1.518e-12       & 1.020e-15       & 1.091e-10       & \bad 5.052e-01  & 1.823e-11       & 1.039e-15       & 1.485e-16 \\
    7  & 0.959 & (0, 1)      & 4.075e-12       & 1.820e-15       & 2.025e-10       & \bad 9.031e-01  & 3.259e-11       & 5.185e-16       & 4.227e-17 \\
    8  & 0.959 & (-1, 1)     & 2.689e-11       & 1.859e-15       & 2.990e-11       & 4.527e-11       & 2.670e-16       & 2.239e-16       & 1.371e-16 \\
    9  & 0.959 & (1, 1)      & \good 5.183e-01 & 7.382e-15       & \bad 5.762e-01  & 1.067e-10       & 7.061e-11       & 3.101e-15       & 2.859e-15 \\
    10 & 1.216 & (-1, 1+1/4) & 6.510e-17       & 6.019e-11       & 1.042e-16       & 1.921e-15       & 3.178e-16       & 3.843e-16       & 1.223e-16 \\
    11 & 1.216 & (-1, 1+1/4) & 5.307e-16       & 6.865e-11       & 7.120e-16       & 1.391e-15       & 3.005e-16       & 1.358e-16       & 8.285e-17 \\
    12 & 1.216 & (-1, 1+1/4) & 4.249e-16       & 2.416e-11       & 8.148e-16       & 4.073e-15       & 2.484e-16       & 1.272e-16       & 1.209e-16 \\
    13 & 1.216 & (-1, 1+1/4) & 2.455e-16       & 8.021e-12       & 4.521e-16       & 2.631e-16       & 2.976e-16       & 2.922e-16       & 2.234e-16 \\
    14 & 1.216 & (1, 1+1/4)  & 6.509e-15       & \good 4.781e-01 & 2.564e-15       & 2.758e-15       & 2.587e-16       & 2.079e-16       & 3.778e-16 \\
    15 & 1.216 & (1, 1+1/4)  & 8.550e-15       & \good 7.141e-01 & 3.372e-15       & 1.789e-15       & 2.780e-16       & 1.086e-16       & 3.907e-16 \\
    16 & 1.216 & (1, 1+1/4)  & 4.634e-15       & \good 5.123e-01 & 2.874e-15       & 3.657e-15       & 1.700e-16       & 6.235e-17       & 3.741e-16 \\
    17 & 1.216 & (1, 1+1/4)  & 3.203e-15       & \good 3.976e-01 & 2.022e-15       & 1.913e-15       & 2.805e-16       & 1.757e-16       & 2.675e-16 \\
    18 & 1.919 & (0, 2)      & 2.812e-16       & 4.137e-16       & 7.801e-11       & \good 3.559e-01 & 1.284e-11       & 7.785e-16       & 9.478e-17 \\
    19 & 2.000 & (-1, 2)     & 1.968e-12       & 6.976e-16       & 9.505e-13       & 2.307e-16       & 4.849e-12       & 4.178e-15       & 2.715e-15 \\
    20 & 2.000 & (-1, 2)     & 8.242e-12       & 8.128e-17       & 4.844e-12       & 3.549e-17       & 3.881e-12       & 7.392e-16       & 6.227e-16 \\
    21 & 2.000 & (-1, 2)     & 1.450e-11       & 4.031e-17       & 1.368e-11       & 1.027e-16       & 7.315e-12       & 5.798e-16       & 1.136e-15 \\
    22 & 2.000 & (-1, 2)     & 1.831e-11       & 8.237e-17       & 1.993e-12       & 2.046e-16       & 5.108e-12       & 9.647e-16       & 1.998e-16 \\
    23 & 2.000 & (1, 2)      & \bad 4.648e-01  & 3.917e-15       & \good 3.806e-01 & 6.492e-11       & 4.055e-11       & 2.128e-16       & 1.392e-15 \\
    24 & 2.000 & (1, 2)      & \bad 1.437e-01  & 1.826e-15       & \good 6.135e-01 & 1.064e-10       & 5.895e-11       & 1.785e-15       & 9.359e-16 \\
    25 & 2.000 & (1, 2)      & \bad 3.164e-01  & 3.711e-15       & \good 4.870e-01 & 7.362e-11       & 2.781e-11       & 9.552e-16       & 2.343e-15 \\
    26 & 2.000 & (1, 2)      & \bad 2.899e-01  & 3.117e-15       & \good 1.268e-01 & 1.182e-11       & 2.874e-12       & 2.934e-15       & 1.407e-15 \\
    27 & 2.000 & (-2, 2)     & 8.537e-12       & 4.170e-16       & 3.216e-12       & 4.579e-16       & 5.014e-12       & 1.917e-15       & 2.484e-15 \\
    28 & 2.000 & (-2, 2)     & 1.645e-11       & 1.588e-16       & 1.545e-11       & 3.429e-16       & 1.537e-11       & 6.567e-16       & 8.569e-16 \\
    29 & 2.000 & (-2, 2)     & 2.164e-11       & 1.943e-16       & 2.632e-11       & 4.852e-17       & 1.764e-11       & 2.056e-16       & 1.091e-15 \\
    30 & 2.000 & (-2, 2)     & 1.067e-11       & 2.014e-17       & 2.818e-12       & 4.102e-16       & 1.128e-12       & 4.001e-16       & 4.967e-16 \\
    31 & 2.000 & (2, 2)      & 1.044e-11       & 2.259e-16       & 7.561e-11       & 2.277e-11       & \good 3.689e-01 & 1.056e-15       & 4.923e-16 \\
    32 & 2.000 & (2, 2)      & 2.492e-11       & 7.301e-17       & 6.679e-11       & 2.410e-11       & \good 3.904e-01 & 6.301e-16       & 2.271e-15 \\
    33 & 2.000 & (2, 2)      & 1.134e-11       & 2.059e-16       & 3.484e-11       & 4.293e-12       & \good 6.957e-02 & 9.089e-16       & 2.796e-15 \\
    34 & 2.000 & (2, 2)      & 3.939e-12       & 6.725e-17       & 5.227e-11       & 1.975e-11       & \good 3.200e-01 & 2.253e-16       & 2.540e-15 \\
    35 & 2.195 & (0, 2+1/4)  & 2.053e-15       & 2.327e-16       & 1.979e-15       & 1.877e-15       & 1.368e-15       & \good 3.696e-01 & 2.602e-12 \\
    36 & 2.195 & (0, 2+1/4)  & 6.288e-16       & 3.234e-16       & 8.580e-16       & 1.791e-15       & 3.288e-16       & \good 5.306e-02 & 1.510e-11 \\
    37 & 2.195 & (0, 2+1/4)  & 1.745e-15       & 3.589e-16       & 1.138e-15       & 3.367e-15       & 1.055e-15       & \good 2.347e-01 & 7.151e-12 \\
    38 & 2.195 & (0, 2+1/4)  & 1.299e-15       & 1.713e-16       & 1.168e-15       & 9.117e-16       & 5.968e-16       & \good 1.773e-01 & 7.317e-12 \\
    39 & 2.195 & (0, 2+1/4)  & 1.242e-15       & 1.738e-16       & 3.561e-16       & 6.054e-16       & 5.048e-16       & \good 9.924e-02 & 8.668e-12 \\
    40 & 2.195 & (0, 2+1/4)  & 3.270e-16       & 8.875e-17       & 5.018e-16       & 3.345e-16       & 2.662e-16       & \good 1.430e-01 & 1.187e-11 \\
    41 & 2.195 & (0, 2+1/4)  & 3.796e-17       & 1.624e-16       & 1.758e-16       & 1.203e-15       & 1.682e-16       & \good 3.495e-01 & 1.165e-11 \\
    42 & 2.195 & (0, 2+1/4)  & 2.522e-17       & 3.743e-16       & 9.655e-17       & 6.641e-16       & 1.456e-16       & \good 9.315e-02 & 2.102e-11 \\
    43 & 2.195 & (-2, 2+1/4) & 1.138e-15       & 5.302e-16       & 8.395e-16       & 3.795e-16       & 6.918e-16       & 2.725e-12       & 2.541e-12 \\
    44 & 2.195 & (-2, 2+1/4) & 1.235e-15       & 3.312e-16       & 1.542e-15       & 3.598e-17       & 5.377e-16       & 1.180e-12       & 3.255e-12 \\
    45 & 2.195 & (2, 2+1/4)  & 1.489e-15       & 1.485e-16       & 1.112e-15       & 7.241e-16       & 2.307e-15       & 2.999e-11       & \good  4.081e-01 \\
    46 & 2.195 & (2, 2+1/4)  & 1.675e-15       & 7.517e-17       & 1.038e-15       & 6.622e-16       & 8.062e-16       & 2.772e-11       & \good  1.787e-01 \\
    47 & 2.377 & (-2, 2+1/4) & 4.418e-16       & 3.444e-16       & 3.947e-16       & 6.947e-17       & 1.292e-16       & 1.086e-15       & 3.550e-12 \\
    48 & 2.377 & (-2, 2+1/4) & 1.031e-15       & 1.532e-16       & 1.239e-15       & 4.650e-16       & 4.607e-16       & 8.862e-16       & 2.474e-12 \\
    49 & 2.377 & (-2, 2+1/4) & 6.110e-16       & 9.260e-17       & 2.389e-16       & 8.948e-17       & 9.831e-16       & 1.028e-15       & 5.179e-12 \\
    50 & 2.377 & (-2, 2+1/4) & 1.323e-15       & 1.048e-17       & 4.112e-16       & 4.093e-17       & 7.262e-16       & 1.550e-15       & 2.151e-12 \\
    51 & 2.377 & (2, 2+1/4)  & 1.052e-15       & 2.213e-16       & 1.268e-15       & 9.389e-16       & 2.294e-15       & 5.728e-11       & \good 3.248e-01 \\
    52 & 2.377 & (2, 2+1/4)  & 6.045e-16       & 8.078e-17       & 1.039e-15       & 9.054e-16       & 6.901e-16       & 2.348e-11       & \good 2.142e-01 \\
    53 & 2.377 & (2, 2+1/4)  & 8.075e-16       & 1.878e-16       & 2.008e-15       & 5.722e-16       & 1.860e-15       & 2.249e-11       & \good 1.586e-01 \\
    54 & 2.377 & (2, 2+1/4)  & 2.023e-15       & 2.498e-16       & 9.265e-16       & 4.246e-16       & 9.182e-16       & 1.254e-11       & \good 1.564e-01 \\
    \bottomrule
  \end{tabular}
  \caption{\M{\phi_\beta}}
  \label{tab:dimer_jm1}
\end{table}

\begin{table}[htb]
  \centering\small
  \def\M#1{$\mel{\phi_\alpha}{\bar{J}_{-1}}{#1}$}
  \begin{tabular}{*{10}{c}}
    \toprule
    $\ket{\phi_\alpha}$ & $\Delta_\alpha$ & $(s_\alpha, \Delta^{\text{exact}}_\alpha)$ & \M{1} & \M{2} & \M{4} & \M{8} & \M{9} & \M{10} & \M{14} \\
    \midrule
    1  & 0.000 & (0, 0)      & 3.020e-16       & 5.799e-17       & 3.742e-11       & 1.430e-11       & \bad 2.318e-01  & 2.456e-16       & 1.159e-14 \\
    2  & 0.238 & (0, 1/4)    & 1.135e-16       & 1.266e-16       & 5.385e-16       & 5.564e-16       & 7.680e-15       & 3.914e-11       & \bad 4.483e-01 \\
    3  & 0.238 & (0, 1/4)    & 3.490e-16       & 5.037e-16       & 1.165e-15       & 1.463e-15       & 4.741e-15       & 7.515e-11       & \bad 5.998e-01 \\
    4  & 0.959 & (0, 1)      & 9.915e-11       & 3.506e-16       & 9.197e-11       & 1.378e-11       & \bad 2.232e-01  & 1.913e-16       & 1.682e-15 \\
    5  & 0.959 & (0, 1)      & 1.805e-11       & 4.414e-15       & 9.393e-11       & 3.324e-11       & \bad 5.386e-01  & 4.190e-16       & 4.006e-15 \\
    6  & 0.959 & (0, 1)      & 2.372e-12       & 1.384e-15       & 9.074e-11       & 3.556e-11       & \bad 5.761e-01  & 3.588e-16       & 3.894e-15 \\
    7  & 0.959 & (0, 1)      & 6.623e-12       & 1.630e-15       & 1.102e-10       & 3.932e-11       & \bad 6.371e-01  & 3.628e-16       & 3.257e-15 \\
    8  & 0.959 & (-1, 1)     & \good 5.183e-01 & 3.244e-15       & \bad 6.618e-01  & 1.461e-10       & 5.360e-11       & 3.492e-15       & 3.110e-15 \\
    9  & 0.959 & (1, 1)      & 2.224e-11       & 7.495e-16       & 2.840e-11       & 5.159e-16       & 1.825e-11       & 1.598e-16       & 4.967e-16 \\
    10 & 1.216 & (-1, 1+1/4) & 4.985e-15       & \good 3.214e-01 & 1.872e-15       & 7.236e-16       & 3.155e-15       & 1.660e-16       & 7.968e-17 \\
    11 & 1.216 & (-1, 1+1/4) & 2.734e-15       & \good 5.641e-01 & 2.131e-15       & 5.335e-16       & 2.215e-15       & 7.069e-16       & 1.585e-16 \\
    12 & 1.216 & (-1, 1+1/4) & 2.698e-15       & \good 3.587e-01 & 8.678e-16       & 6.764e-16       & 3.653e-15       & 5.304e-16       & 3.257e-16 \\
    13 & 1.216 & (-1, 1+1/4) & 9.450e-15       & \good 3.931e-01 & 4.147e-15       & 1.293e-16       & 1.070e-15       & 4.191e-16       & 9.056e-17 \\
    14 & 1.216 & (1, 1+1/4)  & 5.947e-18       & 4.593e-11       & 1.085e-16       & 3.680e-16       & 3.192e-15       & 1.567e-16       & 3.594e-17 \\
    15 & 1.216 & (1, 1+1/4)  & 7.334e-17       & 4.432e-11       & 3.793e-17       & 6.033e-16       & 1.814e-15       & 9.617e-17       & 1.092e-16 \\
    16 & 1.216 & (1, 1+1/4)  & 1.002e-16       & 1.975e-12       & 1.814e-16       & 4.179e-16       & 3.739e-15       & 1.424e-16       & 1.719e-16 \\
    17 & 1.216 & (1, 1+1/4)  & 2.789e-16       & 1.254e-11       & 3.339e-17       & 7.064e-16       & 1.273e-15       & 5.418e-17       & 2.423e-16 \\
    18 & 1.919 & (0, 2)      & 1.419e-16       & 6.304e-16       & 4.830e-11       & 1.846e-11       & \good 2.992e-01 & 4.875e-16       & 1.008e-15 \\
    19 & 2.000 & (-1, 2)     & \bad 3.999e-01  & 3.270e-15       & \good 3.811e-02 & 3.825e-11       & 9.864e-12       & 1.938e-15       & 3.278e-15 \\
    20 & 2.000 & (-1, 2)     & \bad 1.835e-01  & 2.070e-15       & \good 2.333e-01 & 3.843e-11       & 2.003e-11       & 3.927e-15       & 4.149e-15 \\
    21 & 2.000 & (-1, 2)     & \bad 2.438e-01  & 1.934e-15       & \good 2.347e-01 & 2.554e-11       & 1.580e-11       & 2.017e-15       & 1.642e-15 \\
    22 & 2.000 & (-1, 2)     & \bad 4.389e-01  & 5.504e-15       & \good 1.047e-01 & 4.353e-11       & 1.976e-11       & 2.228e-15       & 3.253e-15 \\
    23 & 2.000 & (1, 2)      & 1.002e-11       & 2.479e-17       & 5.180e-12       & 5.637e-12       & 1.646e-16       & 9.017e-16       & 1.216e-15 \\
    24 & 2.000 & (1, 2)      & 2.807e-12       & 2.346e-16       & 2.478e-12       & 1.427e-11       & 8.927e-17       & 7.120e-16       & 2.025e-15 \\
    25 & 2.000 & (1, 2)      & 1.079e-11       & 3.719e-16       & 6.176e-12       & 5.451e-12       & 2.984e-17       & 1.597e-15       & 9.887e-16 \\
    26 & 2.000 & (1, 2)      & 2.358e-11       & 8.030e-17       & 7.652e-12       & 6.347e-12       & 5.828e-16       & 1.393e-15       & 1.055e-15 \\
    27 & 2.000 & (-2, 2)     & 1.140e-11       & 5.040e-16       & 1.463e-10       & \good 6.736e-01 & 2.431e-11       & 2.067e-15       & 1.468e-15 \\
    28 & 2.000 & (-2, 2)     & 1.313e-11       & 1.233e-16       & 6.710e-11       & \good 3.379e-01 & 1.219e-11       & 1.927e-15       & 5.313e-16 \\
    29 & 2.000 & (-2, 2)     & 1.953e-11       & 2.725e-16       & 6.582e-12       & \good 5.926e-02 & 2.138e-12       & 1.027e-15       & 2.286e-16 \\
    30 & 2.000 & (-2, 2)     & 3.216e-11       & 4.221e-17       & 2.207e-11       & \good 1.419e-01 & 5.118e-12       & 2.223e-15       & 2.871e-16 \\
    31 & 2.000 & (2, 2)      & 2.261e-12       & 3.761e-16       & 1.231e-12       & 1.064e-11       & 5.813e-16       & 9.305e-16       & 9.373e-16 \\
    32 & 2.000 & (2, 2)      & 3.628e-13       & 1.581e-16       & 4.027e-12       & 3.708e-12       & 2.810e-16       & 1.290e-15       & 5.026e-16 \\
    33 & 2.000 & (2, 2)      & 5.142e-12       & 1.018e-17       & 2.166e-12       & 1.184e-12       & 3.061e-16       & 2.051e-15       & 6.268e-16 \\
    34 & 2.000 & (2, 2)      & 6.406e-12       & 2.737e-17       & 1.730e-12       & 7.993e-13       & 1.112e-16       & 2.069e-15       & 3.574e-16 \\
    35 & 2.195 & (0, 2+1/4)  & 2.271e-15       & 3.340e-16       & 1.223e-15       & 3.944e-15       & 1.028e-15       & 9.913e-12       & \good 2.836e-01 \\
    36 & 2.195 & (0, 2+1/4)  & 1.209e-15       & 3.093e-16       & 8.933e-16       & 1.293e-15       & 8.158e-16       & 2.570e-11       & \good 1.279e-01 \\
    37 & 2.195 & (0, 2+1/4)  & 3.761e-16       & 1.995e-16       & 2.839e-16       & 1.739e-15       & 1.743e-15       & 1.777e-11       & \good 1.523e-01 \\
    38 & 2.195 & (0, 2+1/4)  & 7.344e-17       & 1.465e-16       & 1.024e-15       & 7.608e-16       & 1.464e-15       & 1.269e-11       & \good 2.161e-01 \\
    39 & 2.195 & (0, 2+1/4)  & 1.450e-15       & 1.452e-16       & 9.658e-16       & 7.077e-16       & 1.262e-15       & 1.628e-11       & \good 1.951e-01 \\
    40 & 2.195 & (0, 2+1/4)  & 1.645e-15       & 1.447e-16       & 1.149e-15       & 4.737e-16       & 7.450e-16       & 9.775e-12       & \good 7.257e-02 \\
    41 & 2.195 & (0, 2+1/4)  & 2.640e-16       & 3.336e-16       & 5.001e-16       & 6.720e-16       & 1.304e-15       & 1.739e-11       & \good 2.373e-01 \\
    42 & 2.195 & (0, 2+1/4)  & 1.071e-16       & 2.901e-16       & 4.304e-16       & 2.360e-16       & 5.700e-16       & 2.373e-11       & \good 2.880e-01 \\
    43 & 2.195 & (-2, 2+1/4) & 1.334e-15       & 2.948e-16       & 1.152e-15       & 2.702e-15       & 3.894e-18       & \good 3.877e-01 & 1.518e-11 \\
    44 & 2.195 & (-2, 2+1/4) & 2.202e-15       & 2.793e-16       & 7.729e-16       & 4.107e-15       & 4.027e-16       & \good 1.493e-01 & 1.477e-11 \\
    45 & 2.195 & (2, 2+1/4)  & 1.482e-15       & 4.563e-16       & 4.938e-16       & 1.865e-15       & 3.565e-17       & 1.042e-12       & 4.851e-13 \\
    46 & 2.195 & (2, 2+1/4)  & 4.905e-16       & 2.675e-16       & 6.223e-16       & 9.047e-16       & 3.614e-17       & 5.295e-12       & 5.308e-16 \\
    47 & 2.377 & (-2, 2+1/4) & 5.851e-16       & 3.386e-17       & 3.655e-16       & 1.372e-15       & 2.725e-16       & \good 2.010e-01 & 2.553e-11 \\
    48 & 2.377 & (-2, 2+1/4) & 5.408e-16       & 1.632e-16       & 6.563e-17       & 1.133e-15       & 6.621e-16       & \good 5.170e-01 & 4.421e-11 \\
    49 & 2.377 & (-2, 2+1/4) & 7.664e-16       & 5.823e-17       & 4.148e-16       & 2.253e-15       & 2.173e-16       & \good 3.372e-01 & 2.652e-11 \\
    50 & 2.377 & (-2, 2+1/4) & 7.657e-16       & 1.805e-16       & 2.843e-16       & 1.822e-15       & 3.796e-16       & \good 3.870e-01 & 4.651e-12 \\
    51 & 2.377 & (2, 2+1/4)  & 2.777e-15       & 2.141e-16       & 1.112e-15       & 1.403e-15       & 3.865e-16       & 2.678e-12       & 2.201e-12 \\
    52 & 2.377 & (2, 2+1/4)  & 8.471e-16       & 4.432e-16       & 3.088e-16       & 4.609e-16       & 4.860e-17       & 8.292e-12       & 2.122e-16 \\
    53 & 2.377 & (2, 2+1/4)  & 1.658e-15       & 6.381e-17       & 9.357e-17       & 5.356e-16       & 1.621e-16       & 7.703e-12       & 6.784e-17 \\
    54 & 2.377 & (2, 2+1/4)  & 9.213e-16       & 1.814e-16       & 3.439e-16       & 3.685e-16       & 2.471e-17       & 1.386e-12       & 1.645e-15 \\
    \bottomrule
  \end{tabular}
  \caption{\M{\phi_\beta}}
  \label{tab:dimer_jbarm1}
\end{table}

\begin{table}[htb]
  \centering\small
  \def\M#1{$\mel{\phi_\alpha}{J_{-2}}{#1}$}
  \def\Mb#1{$\mel{\phi_\alpha}{\bar{J}_{-2}}{#1}$}
  \begin{tabular}{*{10}{c}}
    \toprule
    $\ket{\phi_\alpha}$ & $\Delta_\alpha$ & $(s_\alpha, \Delta^{\text{exact}}_\alpha)$ & \M1 & \Mb1 & \M2 & \Mb2 & \M4 & \Mb4 \\
    \midrule
    1  & 0.000 & (0, 0)      & 2.194e-16       & 3.659e-16       & 1.213e-17       & 1.032e-17       & 2.798e-16      & 2.106e-16 \\
    2  & 0.238 & (0, 1/4)    & 8.377e-19       & 4.856e-17       & 1.364e-16       & 4.728e-16       & 9.702e-17      & 5.544e-17 \\
    3  & 0.238 & (0, 1/4)    & 4.599e-17       & 1.376e-16       & 3.707e-16       & 3.182e-16       & 1.963e-16      & 1.692e-16 \\
    4  & 0.959 & (0, 1)      & 9.406e-17       & 1.472e-16       & 2.741e-17       & 7.702e-17       & 3.837e-16      & 1.160e-16 \\
    5  & 0.959 & (0, 1)      & 1.101e-16       & 2.293e-16       & 7.341e-17       & 5.621e-17       & 7.833e-16      & 3.063e-16 \\
    6  & 0.959 & (0, 1)      & 3.184e-16       & 3.024e-16       & 2.215e-16       & 1.385e-16       & 6.661e-16      & 3.529e-17 \\
    7  & 0.959 & (0, 1)      & 1.401e-16       & 5.457e-16       & 1.898e-16       & 1.231e-16       & 7.434e-17      & 2.547e-16 \\
    8  & 0.959 & (-1, 1)     & 5.993e-17       & 1.192e-16       & 3.856e-17       & 1.080e-16       & 1.575e-16      & 2.826e-12 \\
    9  & 0.959 & (1, 1)      & 1.117e-16       & 1.813e-16       & 1.013e-17       & 1.377e-17       & 4.565e-12      & 1.624e-16 \\
    10 & 1.216 & (-1, 1+1/4) & 9.443e-17       & 1.048e-17       & 2.012e-16       & 2.514e-16       & 2.827e-16      & 8.619e-16 \\
    11 & 1.216 & (-1, 1+1/4) & 7.415e-17       & 3.687e-17       & 2.573e-16       & 1.988e-16       & 3.123e-16      & 7.400e-16 \\
    12 & 1.216 & (-1, 1+1/4) & 3.593e-17       & 1.049e-16       & 2.114e-16       & 4.771e-16       & 3.535e-16      & 1.078e-15 \\
    13 & 1.216 & (-1, 1+1/4) & 2.256e-16       & 1.911e-16       & 2.907e-16       & 5.072e-16       & 3.243e-16      & 1.104e-15 \\
    14 & 1.216 & (1, 1+1/4)  & 4.307e-17       & 1.350e-16       & 1.811e-16       & 2.119e-16       & 3.112e-16      & 2.002e-16 \\
    15 & 1.216 & (1, 1+1/4)  & 7.404e-17       & 2.228e-16       & 1.634e-16       & 2.107e-16       & 3.727e-16      & 2.639e-16 \\
    16 & 1.216 & (1, 1+1/4)  & 4.849e-17       & 1.392e-16       & 3.222e-16       & 3.846e-16       & 2.661e-16      & 1.687e-16 \\
    17 & 1.216 & (1, 1+1/4)  & 1.340e-16       & 1.475e-16       & 2.968e-16       & 2.126e-16       & 4.533e-16      & 2.898e-16 \\
    18 & 1.919 & (0, 2)      & 1.844e-16       & 2.281e-16       & 1.862e-16       & 2.694e-16       & 3.284e-16      & 1.916e-16 \\
    19 & 2.000 & (-1, 2)     & 1.502e-12       & 5.731e-12       & 1.147e-15       & 2.872e-15       & 4.912e-12      & 6.888e-11 \\
    20 & 2.000 & (-1, 2)     & 4.641e-12       & 1.237e-11       & 9.452e-16       & 1.328e-15       & 4.387e-12      & 3.122e-11 \\
    21 & 2.000 & (-1, 2)     & 5.865e-12       & 9.658e-12       & 1.714e-15       & 1.891e-15       & 5.425e-12      & 8.727e-11 \\
    22 & 2.000 & (-1, 2)     & 6.081e-12       & 4.235e-11       & 7.000e-16       & 1.299e-15       & 7.953e-12      & 1.034e-11 \\
    23 & 2.000 & (1, 2)      & 3.906e-12       & 4.488e-12       & 2.224e-15       & 9.620e-16       & 6.344e-11      & 5.522e-12 \\
    24 & 2.000 & (1, 2)      & 2.882e-11       & 8.244e-12       & 1.473e-15       & 5.436e-16       & 1.373e-10      & 5.865e-12 \\
    25 & 2.000 & (1, 2)      & 1.622e-11       & 9.787e-12       & 1.425e-15       & 1.356e-15       & 7.522e-11      & 2.447e-11 \\
    26 & 2.000 & (1, 2)      & 7.050e-12       & 1.439e-11       & 1.606e-15       & 8.611e-16       & 6.315e-11      & 1.006e-11 \\
    27 & 2.000 & (-2, 2)     & 7.211e-12       & \good 3.044e-01 & 1.727e-15       & 2.134e-15       & 5.893e-12      & \bad 5.222e-01 \\
    28 & 2.000 & (-2, 2)     & 1.706e-11       & \good 4.629e-02 & 1.484e-15       & 5.751e-15       & 1.096e-11      & \bad 4.649e-01 \\
    29 & 2.000 & (-2, 2)     & 1.511e-11       & \good 2.115e-01 & 1.451e-15       & 2.826e-15       & 1.075e-11      & \bad 3.456e-01 \\
    30 & 2.000 & (-2, 2)     & 3.824e-12       & \good 6.287e-01 & 7.909e-16       & 9.918e-16       & 3.807e-12      & \bad 2.923e-01 \\
    31 & 2.000 & (2, 2)      & \good 3.380e-01 & 6.555e-12       & 7.619e-16       & 1.541e-15       & \bad 2.352e-01 & 1.286e-11 \\
    32 & 2.000 & (2, 2)      & \good 2.816e-01 & 8.877e-12       & 3.110e-15       & 1.371e-15       & \bad 1.694e-01 & 1.257e-11 \\
    33 & 2.000 & (2, 2)      & \good 2.577e-01 & 1.012e-11       & 4.569e-15       & 9.969e-16       & \bad 2.264e-01 & 2.027e-11 \\
    34 & 2.000 & (2, 2)      & \good 4.637e-01 & 3.614e-12       & 2.901e-15       & 2.480e-15       & \bad 5.672e-01 & 2.018e-12 \\
    35 & 2.195 & (0, 2+1/4)  & 1.167e-15       & 1.828e-15       & 9.615e-13       & 2.382e-12       & 2.581e-15      & 2.690e-15 \\
    36 & 2.195 & (0, 2+1/4)  & 1.305e-15       & 6.678e-16       & 2.791e-13       & 1.038e-12       & 1.031e-15      & 1.240e-15 \\
    37 & 2.195 & (0, 2+1/4)  & 1.047e-15       & 1.135e-15       & 1.271e-12       & 2.231e-12       & 1.554e-15      & 1.661e-15 \\
    38 & 2.195 & (0, 2+1/4)  & 5.541e-16       & 1.705e-16       & 6.295e-13       & 6.343e-13       & 4.878e-16      & 7.357e-16 \\
    39 & 2.195 & (0, 2+1/4)  & 7.794e-16       & 3.391e-16       & 5.345e-13       & 3.914e-13       & 1.329e-16      & 2.473e-16 \\
    40 & 2.195 & (0, 2+1/4)  & 5.086e-16       & 9.840e-16       & 1.668e-13       & 1.307e-13       & 1.170e-15      & 3.583e-16 \\
    41 & 2.195 & (0, 2+1/4)  & 1.193e-16       & 2.020e-16       & 1.325e-13       & 1.266e-13       & 1.753e-16      & 2.733e-16 \\
    42 & 2.195 & (0, 2+1/4)  & 6.604e-17       & 5.515e-17       & 1.889e-14       & 5.218e-14       & 1.103e-16      & 3.927e-16 \\
    43 & 2.195 & (-2, 2+1/4) & 1.019e-15       & 1.238e-15       & 3.150e-12       & \good 4.075e-01 & 9.162e-16      & 2.515e-15 \\
    44 & 2.195 & (-2, 2+1/4) & 4.996e-16       & 1.763e-15       & 2.271e-12       & \good 3.051e-01 & 4.302e-16      & 3.554e-15 \\
    45 & 2.195 & (2, 2+1/4)  & 1.530e-15       & 8.424e-16       & \good 3.537e-01 & 2.683e-12       & 5.932e-16      & 1.291e-15 \\
    46 & 2.195 & (2, 2+1/4)  & 7.470e-16       & 7.818e-16       & \good 3.272e-01 & 2.380e-12       & 3.184e-15      & 1.618e-15 \\
    47 & 2.377 & (-2, 2+1/4) & 2.677e-16       & 5.734e-15       & 7.256e-12       & \good 2.523e-01 & 3.928e-16      & 9.787e-16 \\
    48 & 2.377 & (-2, 2+1/4) & 1.177e-15       & 7.462e-15       & 2.931e-12       & \good 1.915e-01 & 1.809e-16      & 6.705e-16 \\
    49 & 2.377 & (-2, 2+1/4) & 1.971e-15       & 5.454e-15       & 3.323e-12       & \good 4.874e-01 & 1.894e-15      & 1.455e-15 \\
    50 & 2.377 & (-2, 2+1/4) & 1.225e-15       & 6.717e-15       & 2.831e-12       & \good 5.481e-01 & 2.683e-16      & 7.247e-16 \\
    51 & 2.377 & (2, 2+1/4)  & 5.192e-15       & 6.196e-16       & \good 5.129e-01 & 2.238e-12       & 1.318e-15      & 6.241e-16 \\
    52 & 2.377 & (2, 2+1/4)  & 7.118e-16       & 1.705e-15       & \good 1.430e-01 & 1.313e-11       & 1.920e-15      & 5.857e-16 \\
    53 & 2.377 & (2, 2+1/4)  & 4.160e-15       & 1.017e-15       & \good 8.675e-02 & 2.092e-12       & 3.247e-15      & 1.300e-15 \\
    54 & 2.377 & (2, 2+1/4)  & 8.380e-15       & 7.529e-16       & \good 7.333e-01 & 1.266e-12       & 1.726e-15      & 3.195e-16 \\
    \bottomrule
  \end{tabular}
  \caption{\M{\phi_\beta} and \Mb{\phi_\beta}}
  \label{tab:dimer_jm_2_jbarm2}
\end{table}


==> to be submitted to arxiv/isingmel.tex <==
Here we provide the numerical details of the Ising model example discussed in the main text. In this example, we first apply one step of direct blocking as illustrated in Fig.~\ref{fig:rg} to obtain coarse-grained tensor $A=A^{(1)}$ of bond dimension $\chi = 4$ from standard square lattice Ising tensor $A^{(0)}$. More blocking steps or tensor network techniques such as TRG and TNR could be applied to obtain a unit tensor that is closer to the fixed-point, but here we find $A^{(1)}$ is sufficient for the purpose of illustrating our method. Low energy spectrum in terms of conformal spins and scaling dimensions can be obtained by exact diagonalization of transfer matrix on a cylinder, as discussed in last section.

\begin{figure}[ht]
  \centering
  \includegraphics[width=0.5\textwidth]{blocking.pdf}
  \caption{(Top) The $2\times2 \mapsto 1$ coarse-graining procedure. $A^{(s)}$ is made by blocking four copies of $A^{(s-1)}$. (Bottom) The corresponding operator insertion is effected by a square with fewer legs, each with a higher bond dimension.}
  \label{fig:rg}
\end{figure}

Eigenstates $\ket{\phi_T}$ and $\ket{\phi_{\bar{T}}}$ that correspond to energy-momentum tensor $T$ and $\bar{T}$ have conformal spins $s=2$ and $s=-2$. Therefore on a cylinder of $N=4$ sites, these two eigenstates are in fact degenerate. In order to separate these two, one can go back to the original tensor $A^{(0)}$ of bond dimension $\chi=2$ and solve eigenstates from a cylinder of $N=8$ sites of $A^{(0)}$. These eigenstates are then reshaped into four-leg tensors $T$ and $\bar{T}$ with bond dimension $\chi=4$ and subsequently used to construct Virasoro generators $L_n$ and $L_{-n}$ on a cylinder of $N=8$ sites in the coarse-grained lattice of $A$.

We check the property of the lattice Virasoro generators by examining their actions on the low energy eigenstates of transfer matrix on the same cylinder of $N=8$ sites in the coarse-grained lattice. We list the matrix elements $\mel{\phi_\alpha}{L_n}{\phi_\beta}$ and $\mel{\phi_\alpha}{L_{-n}}{\phi_\beta}$ for $n=\pm1, \pm2$ in Table~\ref{tab:ising_lm1}--\ref{tab:ising_lbar2} and illustrate their behaviors on the conformal towers in Fig.~\ref{fig:l1} and~\ref{fig:l2}. In the tables, the matrix elements between states and their correct Virasoro descendant states are highlighted in bold blue, whereas the erroneous matrix elements are marked in pale blue.

\begin{figure}[htb]
  \centering
  \subfloat[$L_{-1}$]{
    \includegraphics[width=0.32\textwidth]{ising_lm1.pdf}
    \label{fig:ising_lm1}}
  \qquad
  \subfloat[$\bar{L}_{-1}$]{
    \includegraphics[width=0.32\textwidth]{ising_lbarm1.pdf}
    \label{fig:ising_lbarm1}}
  \\
  \subfloat[$L_{+1}$]{
    \includegraphics[width=0.32\textwidth]{ising_l1.pdf}
    \label{fig:ising_l1}}
  \qquad
  \subfloat[$\bar{L}_{+1}$]{
    \includegraphics[width=0.32\textwidth]{ising_lbar1.pdf}
    \label{fig:ising_lbar1}}
  \caption{Actions of lattice Virasoro generators $L_{\pm1}$ and $\bar{L}_{\pm1}$ in the low energy subspace of transfer matrix consisting of a row of $N=8$ copies of $A$ with bond dimension $\chi=4$. Corresponding matrix elements are listed in Table~\ref{tab:ising_lm1}--\ref{tab:ising_lbar1}. }
  \label{fig:l1}
\end{figure}

\begin{table}[htb]
  \centering\small
  \def\M#1{$\mel{\phi_\alpha}{L_{-1}}{#1}$}
  \begin{tabular}{*{9}{c}}
    \toprule
    $\ket{\phi_\alpha}$ & $\Delta_\alpha$ & $(s_\alpha, \Delta^{\text{exact}}_\alpha)$ & \M2 & \M3 & \M4 & \M5 & \M6 & \M7 \\
    \midrule
    1  & 0.000 & (0, 0)      & 1.310e-16       & 4.976e-16       & 8.139e-17       & 7.343e-15       & 3.004e-15       & \bad 1.533e-01 \\
    2  & 0.123 & (0, 1/8)    & 5.482e-16       & 1.542e-16       & 7.609e-16       & \bad 8.919e-02  & 1.169e-17       & 9.638e-15 \\
    3  & 0.990 & (0, 1)      & 4.192e-15       & 5.818e-17       & 4.729e-17       & 9.432e-15       & 1.095e-16       & \bad 1.893e-03 \\
    4  & 1.119 & (1, 1+1/8)  & \good 8.968e-01 & 2.961e-15       & 4.735e-16       & 6.775e-16       & 4.944e-17       & 7.085e-17 \\
    5  & 1.119 & (-1, 1+1/8) & 1.112e-14       & 3.685e-16       & 6.305e-17       & 2.599e-17       & 2.711e-17       & 6.328e-17 \\
    6  & 2.000 & (1, 2)      & 3.966e-15       & \good 9.843e-01 & 5.230e-15       & 6.894e-15       & 3.497e-16       & 2.564e-16 \\
    7  & 2.000 & (-1, 2)     & 8.642e-17       & 4.463e-14       & 3.496e-15       & 3.084e-15       & 4.911e-16       & 3.656e-16 \\
    8  & 2.000 & (2, 2)      & 2.381e-17       & 3.123e-14       & 2.406e-15       & 1.607e-15       & \bad 3.717e-03  & 2.814e-16 \\
    9  & 2.000 & (-2, 2)     & 4.239e-17       & 3.613e-14       & 3.492e-15       & 1.603e-15       & 5.501e-16       & 4.390e-16 \\
    10 & 2.114 & (0, 2+1/8)  & 1.263e-16       & 1.149e-15       & 2.273e-14       & \good 9.136e-01 & 8.970e-16       & 2.874e-15 \\
    11 & 2.154 & (2, 2+1/8)  & 7.720e-16       & 9.948e-15       & \good 9.900e-01 & 3.329e-14       & 2.173e-15       & 1.253e-16 \\
    12 & 2.154 & (-2, 2+1/8) & 1.635e-16       & 3.915e-15       & 4.442e-14       & 1.977e-14       & 1.770e-15       & 2.668e-16 \\
    13 & 3.010 & (0, 3)      & 3.158e-17       & 2.695e-16       & 1.163e-16       & 3.422e-15       & 2.371e-14       & \good 9.723e-01 \\
    14 & 3.072 & (2, 3)      & 1.452e-16       & 2.926e-16       & 7.395e-16       & 1.135e-15       & \good 9.869e-01 & 9.407e-14 \\
    15 & 3.072 & (-2, 3)     & 1.580e-16       & 6.671e-17       & 8.238e-17       & 1.617e-16       & 3.911e-14       & 2.981e-16 \\
    16 & 3.072 & (3, 3)      & 3.441e-16       & 2.055e-16       & 4.705e-16       & 3.274e-16       & 4.410e-14       & 5.233e-14 \\
    17 & 3.072 & (-3, 3)     & 2.798e-16       & 3.365e-16       & 7.630e-17       & 9.554e-17       & 1.181e-14       & 2.835e-16 \\
    18 & 3.149 & (1, 3+1/8)  & \bad 2.156e-02  & 1.770e-15       & 3.732e-16       & 1.193e-16       & 2.812e-15       & 4.651e-15 \\
    19 & 3.149 & (-1, 3+1/8) & 1.457e-16       & 6.784e-17       & 4.529e-16       & 7.500e-17       & 6.743e-15       & 7.331e-16 \\
    20 & 3.149 & (3, 3+1/8)  & 5.871e-16       & 1.802e-16       & 1.424e-16       & 6.058e-16       & 4.553e-15       & 1.439e-15 \\
    21 & 3.149 & (-3, 3+1/8) & 1.086e-16       & 2.352e-16       & 2.470e-16       & 4.864e-16       & 2.529e-15       & 5.788e-16 \\
    22 & 3.277 & (3, 3+1/8)  & 5.969e-16       & 1.829e-16       & 3.332e-16       & 8.247e-16       & 4.104e-15       & 7.880e-15 \\
    23 & 3.277 & (-3, 3+1/8) & 3.814e-16       & 1.512e-16       & 1.246e-16       & 4.115e-16       & 2.339e-15       & 2.500e-16 \\
    24 & 4.000 & (0, 4)      & 3.229e-17       & 3.479e-16       & 1.744e-16       & 2.768e-15       & 7.413e-16       & \bad 3.735e-03 \\
    \bottomrule
  \end{tabular}
  \caption{\M{\phi_\beta}}
  \label{tab:ising_lm1}
\end{table}

\begin{table}[htb]
  \centering\small
  \def\M#1{$\mel{\phi_\alpha}{\bar{L}_{-1}}{#1}$}
  \begin{tabular}{*{9}{c}}
    \toprule
    $\ket{\phi_\alpha}$ & $\Delta_\alpha$ & $(s_\alpha, \Delta^{\text{exact}}_\alpha)$ & \M2 & \M3 & \M4 & \M5 & \M6 & \M7 \\
    \midrule
    1  & 0.000 & (0, 0)      & 1.310e-16        & 4.976e-16        & 7.343e-15        & 8.139e-17        & \bad 1.533e-01   & 3.004e-15 \\
    2  & 0.123 & (0, 1/8)    & 5.482e-16        & 1.542e-16        & \bad 8.919e-02   & 7.609e-16        & 9.638e-15        & 1.169e-17 \\
    3  & 0.990 & (0, 1)      & 4.192e-15        & 5.818e-17        & 9.432e-15        & 4.729e-17        & \bad 1.893e-03   & 1.095e-16 \\
    4  & 1.119 & (1, 1+1/8)  & 1.112e-14        & 3.685e-16        & 2.599e-17        & 6.305e-17        & 6.328e-17        & 2.711e-17 \\
    5  & 1.119 & (-1, 1+1/8) & \good  8.968e-01 & 2.961e-15        & 6.775e-16        & 4.735e-16        & 7.085e-17        & 4.944e-17 \\
    6  & 2.000 & (1, 2)      & 8.642e-17        & 4.463e-14        & 3.084e-15        & 3.496e-15        & 3.656e-16        & 4.911e-16 \\
    7  & 2.000 & (-1, 2)     & 3.966e-15        & \good  9.843e-01 & 6.894e-15        & 5.230e-15        & 2.564e-16        & 3.497e-16 \\
    8  & 2.000 & (2, 2)      & 4.239e-17        & 3.613e-14        & 1.603e-15        & 3.492e-15        & 4.390e-16        & 5.501e-16 \\
    9  & 2.000 & (-2, 2)     & 2.381e-17        & 3.123e-14        & 1.607e-15        & 2.406e-15        & 2.814e-16        & \bad 3.717e-03 \\
    10 & 2.114 & (0, 2+1/8)  & 1.263e-16        & 1.149e-15        & \good  9.136e-01 & 2.273e-14        & 2.874e-15        & 8.970e-16 \\
    11 & 2.154 & (2, 2+1/8)  & 1.635e-16        & 3.915e-15        & 1.977e-14        & 4.442e-14        & 2.668e-16        & 1.770e-15 \\
    12 & 2.154 & (-2, 2+1/8) & 7.720e-16        & 9.948e-15        & 3.329e-14        & \good  9.900e-01 & 1.253e-16        & 2.173e-15 \\
    13 & 3.010 & (0, 3)      & 3.158e-17        & 2.695e-16        & 3.422e-15        & 1.163e-16        & \good  9.723e-01 & 2.371e-14 \\
    14 & 3.072 & (2, 3)      & 1.580e-16        & 6.671e-17        & 1.617e-16        & 8.238e-17        & 2.981e-16        & 3.911e-14 \\
    15 & 3.072 & (-2, 3)     & 1.452e-16        & 2.926e-16        & 1.135e-15        & 7.395e-16        & 9.407e-14        & \good  9.869e-01 \\
    16 & 3.072 & (3, 3)      & 2.798e-16        & 3.365e-16        & 9.554e-17        & 7.630e-17        & 2.835e-16        & 1.181e-14 \\
    17 & 3.072 & (-3, 3)     & 3.441e-16        & 2.055e-16        & 3.274e-16        & 4.705e-16        & 5.233e-14        & 4.410e-14 \\
    18 & 3.149 & (1, 3+1/8)  & 1.457e-16        & 6.784e-17        & 7.500e-17        & 4.529e-16        & 7.331e-16        & 6.743e-15 \\
    19 & 3.149 & (-1, 3+1/8) & \bad 2.156e-02   & 1.770e-15        & 1.193e-16        & 3.732e-16        & 4.651e-15        & 2.812e-15 \\
    20 & 3.149 & (3, 3+1/8)  & 1.086e-16        & 2.352e-16        & 4.864e-16        & 2.470e-16        & 5.788e-16        & 2.529e-15 \\
    21 & 3.149 & (-3, 3+1/8) & 5.871e-16        & 1.802e-16        & 6.058e-16        & 1.424e-16        & 1.439e-15        & 4.553e-15 \\
    22 & 3.277 & (3, 3+1/8)  & 3.814e-16        & 1.512e-16        & 4.115e-16        & 1.246e-16        & 2.500e-16        & 2.339e-15 \\
    23 & 3.277 & (-3, 3+1/8) & 5.969e-16        & 1.829e-16        & 8.247e-16        & 3.332e-16        & 7.880e-15        & 4.104e-15 \\
    24 & 4.000 & (0, 4)      & 3.229e-17        & 3.479e-16        & 2.768e-15        & 1.744e-16        & \bad 3.735e-03   & 7.413e-16 \\
    \bottomrule
  \end{tabular}
  \caption{\M{\phi_\beta}}
  \label{tab:ising_lbarm1}
\end{table}

\begin{table}[htb]
  \centering\small
  \def\M#1{$\mel{\phi_\alpha}{L_{+1}}{#1}$}
  \makebox[0pt]{
    \begin{tabular}{*{12}{c}}
      \toprule
      $\ket{\phi_\alpha}$ & $\Delta_\alpha$ & $(s_\alpha, \Delta^{\text{exact}}_\alpha)$ & \M2 & \M3 & \M4 & \M5 & \M6 & \M7 & \M8 & \M9 & \M{10} \\
      \midrule
      1  & 0.000 & (0, 0)      & 8.578e-18      & 2.446e-16      & 2.604e-15       & 6.263e-18      & \bad 7.686e-03  & 3.004e-15      & 2.334e-15      & 1.933e-15      & 1.955e-16 \\
      2  & 0.123 & (0, 1/8)    & 1.552e-16      & 1.161e-14      & \good 9.555e-01 & 3.338e-14      & 4.367e-15       & 5.268e-16      & 1.785e-16      & 2.330e-16      & 1.878e-16 \\
      3  & 0.990 & (0, 1)      & 2.477e-16      & 2.052e-16      & 3.966e-15       & 1.351e-15      & \good 9.921e-01 & 3.729e-13      & 3.098e-13      & 2.601e-13      & 3.469e-15 \\
      4  & 1.119 & (1, 1+1/8)  & 5.814e-16      & 2.309e-16      & 7.517e-16       & 1.113e-15      & 7.151e-15       & 3.756e-14      & 3.285e-14      & 3.384e-14      & 9.396e-14 \\
      5  & 1.119 & (-1, 1+1/8) & \bad 4.909e-02 & 1.219e-14      & 8.994e-16       & 2.158e-16      & 2.381e-15       & 8.371e-15      & 5.368e-15      & 3.924e-15      & \good 9.454e-01 \\
      6  & 2.000 & (1, 2)      & 1.707e-17      & 7.965e-17      & 6.223e-17       & 9.033e-17      & 1.482e-16       & 1.990e-15      & \bad 3.293e-02 & 1.477e-15      & 2.462e-15 \\
      7  & 2.000 & (-1, 2)     & 4.645e-15      & \bad 3.095e-03 & 4.456e-17       & 1.054e-16      & 6.059e-17       & 5.274e-16      & 2.041e-15      & 7.986e-16      & 3.635e-15 \\
      8  & 2.000 & (2, 2)      & 7.978e-18      & 4.242e-16      & 5.599e-17       & 4.756e-17      & 7.192e-16       & 4.693e-16      & 9.823e-16      & 6.746e-16      & 9.167e-16 \\
      9  & 2.000 & (-2, 2)     & 1.314e-17      & 3.184e-16      & 4.905e-17       & 6.633e-15      & 8.610e-16       & \bad 3.055e-02 & 2.679e-15      & 6.948e-16      & 1.862e-17 \\
      10 & 2.114 & (0, 2+1/8)  & 2.846e-16      & 1.943e-16      & \bad 2.048e-02  & 7.711e-16      & 1.396e-15       & 7.353e-16      & 2.907e-16      & 2.730e-16      & 3.822e-16 \\
      11 & 2.154 & (2, 2+1/8)  & 1.532e-16      & 1.199e-16      & 3.187e-16       & 3.318e-16      & 2.437e-16       & 1.543e-15      & 1.025e-15      & 2.221e-16      & 4.611e-16 \\
      12 & 2.154 & (-2, 2+1/8) & 9.078e-17      & 9.965e-18      & 5.960e-16       & \bad 1.747e-03 & 7.664e-17       & 1.100e-14      & 4.836e-17      & 4.007e-17      & 4.441e-16 \\
      13 & 3.010 & (0, 3)      & 5.616e-18      & 5.907e-17      & 1.641e-15       & 7.723e-17      & \bad 1.303e-03  & 3.840e-16      & 5.947e-16      & 3.836e-16      & 1.136e-16 \\
      14 & 3.072 & (2, 3)      & 7.931e-16      & 4.752e-17      & 7.060e-17       & 6.990e-17      & 1.885e-16       & 4.479e-16      & 3.502e-16      & 2.643e-16      & 7.743e-17 \\
      15 & 3.072 & (-2, 3)     & 5.517e-16      & 1.185e-16      & 4.814e-17       & 2.421e-15      & 1.117e-16       & \bad 7.603e-03 & 3.901e-16      & 3.866e-16      & 5.368e-17 \\
      16 & 3.072 & (3, 3)      & 1.499e-15      & 3.170e-16      & 1.598e-17       & 2.964e-17      & 6.698e-16       & 3.871e-16      & 4.962e-16      & 3.717e-16      & 1.844e-17 \\
      17 & 3.072 & (-3, 3)     & 1.811e-15      & 2.346e-16      & 3.627e-17       & 4.429e-17      & 4.135e-16       & 2.970e-16      & 5.172e-16      & \bad 1.233e-02 & 4.658e-17 \\
      18 & 3.149 & (1, 3+1/8)  & 4.561e-16      & 9.261e-18      & 5.164e-16       & 6.611e-17      & 9.135e-18       & 2.588e-16      & 1.353e-15      & 2.115e-16      & 5.545e-16 \\
      19 & 3.149 & (-1, 3+1/8) & \bad 1.089e-01 & 6.010e-15      & 2.104e-16       & 6.268e-17      & 4.399e-17       & 2.843e-16      & 7.615e-17      & 1.238e-16      & \bad 2.463e-03 \\
      20 & 3.149 & (3, 3+1/8)  & 8.824e-16      & 1.183e-17      & 2.263e-17       & 3.453e-17      & 4.263e-17       & 1.052e-16      & 8.315e-17      & 1.835e-16      & 3.285e-16 \\
      21 & 3.149 & (-3, 3+1/8) & 2.440e-15      & 1.398e-17      & 4.274e-17       & 8.467e-17      & 3.126e-17       & 1.830e-16      & 2.468e-16      & 4.537e-15      & 6.787e-16 \\
      22 & 3.277 & (3, 3+1/8)  & 4.873e-16      & 6.136e-17      & 1.360e-16       & 1.070e-16      & 1.031e-16       & 6.228e-16      & 4.779e-16      & 3.234e-16      & 5.780e-16 \\
      23 & 3.277 & (-3, 3+1/8) & 1.049e-15      & 2.730e-17      & 2.764e-16       & 1.366e-16      & 3.310e-17       & 1.044e-16      & 1.319e-16      & 1.019e-15      & 3.057e-16 \\
      24 & 4.000 & (0, 4)      & 3.973e-17      & 1.041e-16      & 1.372e-15       & 1.821e-16      & \bad 1.508e-02  & 5.663e-15      & 4.731e-15      & 3.961e-15      & 1.292e-16 \\
      \bottomrule
    \end{tabular}
  }
  \caption{\M{\phi_\beta}}
  \label{tab:ising_l1}
\end{table}

\begin{table}[htb]
  \centering\small
  \def\M#1{$\mel{\phi_\alpha}{\bar{L}_{+1}}{#1}$}
  \makebox[0pt]{
    \begin{tabular}{*{12}{c}}
      \toprule
      $\ket{\phi_\alpha}$ & $\Delta_\alpha$ & $(s_\alpha, \Delta^{\text{exact}}_\alpha)$ & \M2 & \M3 & \M4 & \M5 & \M6 & \M7 & \M8 & \M9 & \M{10} \\
      \midrule
      1  & 0.000 & (0, 0)      & 8.578e-18      & 2.446e-16      & 6.263e-18      & 2.604e-15       & 3.004e-15      & \bad 7.686e-03  & 1.933e-15      & 2.334e-15      & 1.955e-16 \\
      2  & 0.123 & (0, 1/8)    & 1.552e-16      & 1.161e-14      & 3.338e-14      & \good 9.555e-01 & 5.268e-16      & 4.367e-15       & 2.330e-16      & 1.785e-16      & 1.878e-16 \\
      3  & 0.990 & (0, 1)      & 2.477e-16      & 2.052e-16      & 1.351e-15      & 3.966e-15       & 3.729e-13      & \good 9.921e-01 & 2.601e-13      & 3.098e-13      & 3.469e-15 \\
      4  & 1.119 & (1, 1+1/8)  & \bad 4.909e-02 & 1.219e-14      & 2.158e-16      & 8.994e-16       & 8.371e-15      & 2.381e-15       & 3.924e-15      & 5.368e-15      & \good 9.454e-01 \\
      5  & 1.119 & (-1, 1+1/8) & 5.814e-16      & 2.309e-16      & 1.113e-15      & 7.517e-16       & 3.756e-14      & 7.151e-15       & 3.384e-14      & 3.285e-14      & 9.396e-14 \\
      6  & 2.000 & (1, 2)      & 4.645e-15      & \bad 3.095e-03 & 1.054e-16      & 4.456e-17       & 5.274e-16      & 6.059e-17       & 7.986e-16      & 2.041e-15      & 3.635e-15 \\
      7  & 2.000 & (-1, 2)     & 1.707e-17      & 7.965e-17      & 9.033e-17      & 6.223e-17       & 1.990e-15      & 1.482e-16       & 1.477e-15      & \bad 3.293e-02 & 2.462e-15 \\
      8  & 2.000 & (2, 2)      & 1.314e-17      & 3.184e-16      & 6.633e-15      & 4.905e-17       & \bad 3.055e-02 & 8.610e-16       & 6.948e-16      & 2.679e-15      & 1.862e-17 \\
      9  & 2.000 & (-2, 2)     & 7.978e-18      & 4.242e-16      & 4.756e-17      & 5.599e-17       & 4.693e-16      & 7.192e-16       & 6.746e-16      & 9.823e-16      & 9.167e-16 \\
      10 & 2.114 & (0, 2+1/8)  & 2.846e-16      & 1.943e-16      & 7.711e-16      & \bad 2.048e-02  & 7.353e-16      & 1.396e-15       & 2.730e-16      & 2.907e-16      & 3.822e-16 \\
      11 & 2.154 & (2, 2+1/8)  & 9.078e-17      & 9.965e-18      & \bad 1.747e-03 & 5.960e-16       & 1.100e-14      & 7.664e-17       & 4.007e-17      & 4.836e-17      & 4.441e-16 \\
      12 & 2.154 & (-2, 2+1/8) & 1.532e-16      & 1.199e-16      & 3.318e-16      & 3.187e-16       & 1.543e-15      & 2.437e-16       & 2.221e-16      & 1.025e-15      & 4.611e-16 \\
      13 & 3.010 & (0, 3)      & 5.616e-18      & 5.907e-17      & 7.723e-17      & 1.641e-15       & 3.840e-16      & \bad 1.303e-03  & 3.836e-16      & 5.947e-16      & 1.136e-16 \\
      14 & 3.072 & (2, 3)      & 5.517e-16      & 1.185e-16      & 2.421e-15      & 4.814e-17       & \bad 7.603e-03 & 1.117e-16       & 3.866e-16      & 3.901e-16      & 5.368e-17 \\
      15 & 3.072 & (-2, 3)     & 7.931e-16      & 4.752e-17      & 6.990e-17      & 7.060e-17       & 4.479e-16      & 1.885e-16       & 2.643e-16      & 3.502e-16      & 7.743e-17 \\
      16 & 3.072 & (3, 3)      & 1.811e-15      & 2.346e-16      & 4.429e-17      & 3.627e-17       & 2.970e-16      & 4.135e-16       & \bad 1.233e-02 & 5.172e-16      & 4.658e-17 \\
      17 & 3.072 & (-3, 3)     & 1.499e-15      & 3.170e-16      & 2.964e-17      & 1.598e-17       & 3.871e-16      & 6.698e-16       & 3.717e-16      & 4.962e-16      & 1.844e-17 \\
      18 & 3.149 & (1, 3+1/8)  & \bad 1.089e-01 & 6.010e-15      & 6.268e-17      & 2.104e-16       & 2.843e-16      & 4.399e-17       & 1.238e-16      & 7.615e-17      & \bad 2.463e-03 \\
      19 & 3.149 & (-1, 3+1/8) & 4.561e-16      & 9.261e-18      & 6.611e-17      & 5.164e-16       & 2.588e-16      & 9.135e-18       & 2.115e-16      & 1.353e-15      & 5.545e-16 \\
      20 & 3.149 & (3, 3+1/8)  & 2.440e-15      & 1.398e-17      & 8.467e-17      & 4.274e-17       & 1.830e-16      & 3.126e-17       & 4.537e-15      & 2.468e-16      & 6.787e-16 \\
      21 & 3.149 & (-3, 3+1/8) & 8.824e-16      & 1.183e-17      & 3.453e-17      & 2.263e-17       & 1.052e-16      & 4.263e-17       & 1.835e-16      & 8.315e-17      & 3.285e-16 \\
      22 & 3.277 & (3, 3+1/8)  & 1.049e-15      & 2.730e-17      & 1.366e-16      & 2.764e-16       & 1.044e-16      & 3.310e-17       & 1.019e-15      & 1.319e-16      & 3.057e-16 \\
      23 & 3.277 & (-3, 3+1/8) & 4.873e-16      & 6.136e-17      & 1.070e-16      & 1.360e-16       & 6.228e-16      & 1.031e-16       & 3.234e-16      & 4.779e-16      & 5.780e-16 \\
      24 & 4.000 & (0, 4)      & 3.973e-17      & 1.041e-16      & 1.821e-16      & 1.372e-15       & 5.663e-15      & \bad 1.508e-02  & 3.961e-15      & 4.731e-15      & 1.292e-16 \\
      \bottomrule
    \end{tabular}
  }
  \caption{\M{\phi_\beta}}
  \label{tab:ising_lbar1}
\end{table}

\begin{figure}[htb]
  \centering
  \subfloat[$L_{-2}$]{
    \includegraphics[width=0.32\textwidth]{ising_lm2.pdf}
    \label{fig:ising_lm2}}
  \qquad
  \subfloat[$\bar{L}_{-2}$]{
    \includegraphics[width=0.32\textwidth]{ising_lbarm2.pdf}
    \label{fig:ising_lbarm2}}
  \\
  \subfloat[$L_{+2}$]{
    \includegraphics[width=0.32\textwidth]{ising_l2.pdf}
    \label{fig:ising_l2}}
  \qquad
  \subfloat[$\bar{L}_{+2}$]{
    \includegraphics[width=0.32\textwidth]{ising_lbar2.pdf}
    \label{fig:ising_lbar2}}
  \caption{Actions of lattice $L_{\pm2}$ and $\bar{L}_{\pm2}$ in the low energy subspace of transfer matrix consisting of a row of $N=8$ copies of $A$ with bond dimension $\chi=4$. Corresponding matrix elements are listed in Table~\ref{tab:ising_lm2}--\ref{tab:ising_lbar2}. }
  \label{fig:l2}
\end{figure}

\begin{table}[htb]
  \centering\small
  \def\M#1{$\mel{\phi_\alpha}{L_{-2}}{#1}$}
  \begin{tabular}{*{10}{c}}
    \toprule
    $\ket{\phi_\alpha}$ & $\Delta_\alpha$ & $(s_\alpha, \Delta^{\text{exact}}_\alpha)$ & \M1 & \M2 & \M3 & \M4 & \M5 & \M9 \\
    \midrule
    1  & 0.000 & (0, 0)      & 8.241e-17       & 6.521e-17       & 8.866e-17       & 2.950e-18       & 1.594e-17       & \bad 1.068e-03 \\
    2  & 0.123 & (0, 1/8)    & 6.633e-18       & 2.987e-16       & 6.894e-18       & 3.035e-16       & 7.635e-16       & 7.276e-15 \\
    3  & 0.990 & (0, 1)      & 1.788e-16       & 4.574e-17       & 3.614e-16       & 2.190e-17       & 2.721e-16       & \bad 3.095e-01 \\
    4  & 1.119 & (1, 1+1/8)  & 1.882e-15       & 2.846e-16       & 1.342e-16       & 7.095e-16       & \bad 7.017e-02  & 1.015e-16 \\
    5  & 1.119 & (-1, 1+1/8) & 1.536e-15       & 3.513e-16       & 2.972e-17       & 2.892e-16       & 9.902e-16       & 6.969e-17 \\
    6  & 2.000 & (1, 2)      & 6.049e-13       & 2.695e-15       & 2.314e-16       & 1.085e-16       & 8.067e-15       & 5.437e-15 \\
    7  & 2.000 & (-1, 2)     & 3.870e-13       & 3.393e-15       & 1.097e-17       & 1.124e-16       & 1.497e-16       & 6.186e-16 \\
    8  & 2.000 & (2, 2)      & \good 9.439e-01 & 2.002e-15       & \bad 5.724e-03  & 1.267e-16       & 8.287e-17       & 3.766e-16 \\
    9  & 2.000 & (-2, 2)     & 8.184e-13       & 3.389e-15       & 1.763e-16       & 1.227e-17       & 5.763e-17       & 1.272e-16 \\
    10 & 2.114 & (0, 2+1/8)  & 6.002e-16       & 1.925e-14       & 8.555e-16       & 1.343e-16       & 2.741e-16       & 2.290e-14 \\
    11 & 2.154 & (2, 2+1/8)  & 4.106e-15       & \good 9.608e-01 & 3.152e-15       & 7.502e-16       & 6.615e-16       & 3.385e-16 \\
    12 & 2.154 & (-2, 2+1/8) & 1.414e-15       & 4.282e-14       & 1.790e-15       & 3.127e-16       & 1.774e-16       & 5.431e-17 \\
    13 & 3.010 & (0, 3)      & 8.171e-16       & 1.306e-16       & 6.084e-16       & 5.863e-16       & 1.819e-16       & \bad 1.600e-02 \\
    14 & 3.072 & (2, 3)      & \bad 6.190e-03  & 3.048e-15       & \good 9.837e-01 & 2.157e-15       & 6.658e-15       & 1.768e-16 \\
    15 & 3.072 & (-2, 3)     & 1.383e-15       & 7.996e-17       & 4.043e-14       & 3.138e-15       & 7.003e-15       & 8.258e-16 \\
    16 & 3.072 & (3, 3)      & 1.339e-15       & 3.159e-17       & 2.026e-14       & 3.765e-15       & 1.605e-14       & 4.207e-15 \\
    17 & 3.072 & (-3, 3)     & 1.926e-16       & 7.461e-17       & 1.212e-14       & 2.186e-15       & 1.320e-14       & 3.003e-16 \\
    18 & 3.149 & (1, 3+1/8)  & 1.034e-16       & 3.715e-16       & 2.668e-15       & 9.258e-15       & \good 9.690e-01 & 6.707e-16 \\
    19 & 3.149 & (-1, 3+1/8) & 4.932e-17       & 2.229e-16       & 6.197e-15       & 1.526e-15       & 5.986e-15       & 9.006e-17 \\
    20 & 3.149 & (3, 3+1/8)  & 8.457e-17       & 2.925e-16       & 4.248e-15       & \bad 3.296e-01  & 3.429e-14       & 5.377e-16 \\
    21 & 3.149 & (-3, 3+1/8) & 1.105e-16       & 5.296e-17       & 2.522e-15       & 8.410e-15       & 7.983e-15       & 2.601e-16 \\
    22 & 3.277 & (3, 3+1/8)  & 1.928e-16       & 5.400e-16       & 5.464e-15       & \good 9.288e-01 & 3.894e-14       & 1.614e-15 \\
    23 & 3.277 & (-3, 3+1/8) & 7.712e-17       & 3.538e-16       & 2.324e-15       & 1.382e-14       & 4.187e-15       & 2.780e-16 \\
    24 & 4.000 & (0, 4)      & 1.765e-18       & 1.711e-16       & 7.672e-16       & 1.651e-16       & 6.216e-16       & \good 8.948e-01 \\
    \bottomrule
  \end{tabular}
  \caption{\M{\phi_\beta}}
  \label{tab:ising_lm2}
\end{table}

\begin{table}[htb]
  \centering\small
  \def\M#1{$\mel{\phi_\alpha}{\bar{L}_{-2}}{#1}$}
  \begin{tabular}{*{9}{c}}
    \toprule
    $\ket{\phi_\alpha}$ & $\Delta_\alpha$ & $(s_\alpha, \Delta^{\text{exact}}_\alpha)$ & \M1 & \M2 & \M3 & \M4 & \M5 & \M8 \\
    \midrule
    1  & 0.000 & (0, 0)      & 8.241e-17       & 6.521e-17       & 8.866e-17       & 1.594e-17       & 2.950e-18       & \bad 1.068e-03 \\
    2  & 0.123 & (0, 1/8)    & 6.633e-18       & 2.987e-16       & 6.894e-18       & 7.635e-16       & 3.035e-16       & 7.276e-15 \\
    3  & 0.990 & (0, 1)      & 1.788e-16       & 4.574e-17       & 3.614e-16       & 2.721e-16       & 2.190e-17       & \bad 3.095e-01 \\
    4  & 1.119 & (1, 1+1/8)  & 1.536e-15       & 3.513e-16       & 2.972e-17       & 9.902e-16       & 2.892e-16       & 6.969e-17 \\
    5  & 1.119 & (-1, 1+1/8) & 1.882e-15       & 2.846e-16       & 1.342e-16       & \bad 7.017e-02  & 7.095e-16       & 1.015e-16 \\
    6  & 2.000 & (1, 2)      & 3.870e-13       & 3.393e-15       & 1.097e-17       & 1.497e-16       & 1.124e-16       & 6.186e-16 \\
    7  & 2.000 & (-1, 2)     & 6.049e-13       & 2.695e-15       & 2.314e-16       & 8.067e-15       & 1.085e-16       & 5.437e-15 \\
    8  & 2.000 & (2, 2)      & 8.184e-13       & 3.389e-15       & 1.763e-16       & 5.763e-17       & 1.227e-17       & 1.272e-16 \\
    9  & 2.000 & (-2, 2)     & \good 9.439e-01 & 2.002e-15       & \bad 5.724e-03  & 8.287e-17       & 1.267e-16       & 3.766e-16 \\
    10 & 2.114 & (0, 2+1/8)  & 6.002e-16       & 1.925e-14       & 8.555e-16       & 2.741e-16       & 1.343e-16       & 2.290e-14 \\
    11 & 2.154 & (2, 2+1/8)  & 1.414e-15       & 4.282e-14       & 1.790e-15       & 1.774e-16       & 3.127e-16       & 5.431e-17 \\
    12 & 2.154 & (-2, 2+1/8) & 4.106e-15       & \good 9.608e-01 & 3.152e-15       & 6.615e-16       & 7.502e-16       & 3.385e-16 \\
    13 & 3.010 & (0, 3)      & 8.171e-16       & 1.306e-16       & 6.084e-16       & 1.819e-16       & 5.863e-16       & \bad 1.600e-02 \\
    14 & 3.072 & (2, 3)      & 1.383e-15       & 7.996e-17       & 4.043e-14       & 7.003e-15       & 3.138e-15       & 8.258e-16 \\
    15 & 3.072 & (-2, 3)     & \bad 6.190e-03  & 3.048e-15       & \good 9.837e-01 & 6.658e-15       & 2.157e-15       & 1.768e-16 \\
    16 & 3.072 & (3, 3)      & 1.926e-16       & 7.461e-17       & 1.212e-14       & 1.320e-14       & 2.186e-15       & 3.003e-16 \\
    17 & 3.072 & (-3, 3)     & 1.339e-15       & 3.159e-17       & 2.026e-14       & 1.605e-14       & 3.765e-15       & 4.207e-15 \\
    18 & 3.149 & (1, 3+1/8)  & 4.932e-17       & 2.229e-16       & 6.197e-15       & 5.986e-15       & 1.526e-15       & 9.006e-17 \\
    19 & 3.149 & (-1, 3+1/8) & 1.034e-16       & 3.715e-16       & 2.668e-15       & \good 9.690e-01 & 9.258e-15       & 6.707e-16 \\
    20 & 3.149 & (3, 3+1/8)  & 1.105e-16       & 5.296e-17       & 2.522e-15       & 7.983e-15       & 8.410e-15       & 2.601e-16 \\
    21 & 3.149 & (-3, 3+1/8) & 8.457e-17       & 2.925e-16       & 4.248e-15       & 3.429e-14       & \bad 3.296e-01  & 5.377e-16 \\
    22 & 3.277 & (3, 3+1/8)  & 7.712e-17       & 3.538e-16       & 2.324e-15       & 4.187e-15       & 1.382e-14       & 2.780e-16 \\
    23 & 3.277 & (-3, 3+1/8) & 1.928e-16       & 5.400e-16       & 5.464e-15       & 3.894e-14       & \good 9.288e-01 & 1.614e-15 \\
    24 & 4.000 & (0, 4)      & 1.765e-18       & 1.711e-16       & 7.672e-16       & 6.216e-16       & 1.651e-16       & \good 8.948e-01 \\
    \bottomrule
  \end{tabular}
  \caption{\M{\phi_\beta}}
  \label{tab:ising_lbarm2}
\end{table}

\begin{table}[htb]
  \centering\small
  \def\M#1{$\mel{\phi_\alpha}{L_{+2}}{#1}$}
  \begin{tabular}{*{9}{c}}
    \toprule
    $\ket{\phi_\alpha}$ & $\Delta_\alpha$ & $(s_\alpha, \Delta^{\text{exact}}_\alpha)$ & \M{11} & \M{14} & \M{18} & \M{20} & \M{22} & \M{23} \\
    \midrule
    1  & 0.000 & (0, 0)      & 5.467e-15       & \bad 4.795e-03  & 1.856e-16       & 1.520e-16       & 1.245e-16       & 5.713e-16 \\
    2  & 0.123 & (0, 1/8)    & \good 9.867e-01 & 4.046e-15       & 2.586e-16       & 5.058e-16       & 8.715e-16       & 9.216e-16 \\
    3  & 0.990 & (0, 1)      & 3.940e-15       & \good 9.955e-01 & 1.994e-14       & 1.384e-14       & 1.349e-15       & 1.628e-14 \\
    4  & 1.119 & (1, 1+1/8)  & 6.964e-16       & 2.776e-15       & 3.919e-13       & \good 9.842e-01 & \good 9.962e-01 & 2.353e-12 \\
    5  & 1.119 & (-1, 1+1/8) & 6.594e-16       & 2.919e-15       & \good 9.841e-01 & 4.570e-13       & 4.304e-13       & 1.000e-14 \\
    6  & 2.000 & (1, 2)      & 6.025e-17       & 3.039e-16       & 1.670e-16       & 4.959e-15       & 1.318e-15       & 5.919e-16 \\
    7  & 2.000 & (-1, 2)     & 2.966e-17       & 2.019e-16       & 3.288e-15       & 5.373e-16       & 1.743e-16       & 2.381e-15 \\
    8  & 2.000 & (2, 2)      & 7.495e-17       & 6.037e-16       & 3.122e-16       & 3.257e-16       & 3.502e-16       & 1.903e-15 \\
    9  & 2.000 & (-2, 2)     & 7.485e-17       & 2.251e-16       & 2.593e-16       & 2.083e-16       & 2.246e-16       & 4.436e-16 \\
    10 & 2.114 & (0, 2+1/8)  & \bad 8.935e-04  & 9.438e-16       & 3.131e-16       & 3.338e-16       & 2.725e-16       & 7.598e-16 \\
    11 & 2.154 & (2, 2+1/8)  & 7.313e-16       & 1.787e-16       & 3.496e-16       & 4.773e-16       & 4.931e-16       & 2.210e-15 \\
    12 & 2.154 & (-2, 2+1/8) & 6.331e-16       & 9.592e-17       & 2.916e-16       & 1.403e-16       & 2.540e-16       & 4.221e-16 \\
    13 & 3.010 & (0, 3)      & 1.460e-15       & 1.158e-03       & 6.726e-17       & 5.694e-17       & 8.429e-17       & 1.475e-15 \\
    14 & 3.072 & (2, 3)      & 4.996e-17       & 1.423e-16       & 2.763e-17       & 1.681e-16       & 4.588e-17       & 1.346e-15 \\
    15 & 3.072 & (-2, 3)     & 3.628e-17       & 2.232e-16       & 2.778e-17       & 1.042e-16       & 2.724e-17       & 1.397e-15 \\
    16 & 3.072 & (3, 3)      & 3.601e-17       & 3.837e-16       & 1.870e-16       & 4.195e-16       & 9.056e-17       & 1.606e-14 \\
    17 & 3.072 & (-3, 3)     & 3.907e-17       & 5.139e-16       & 5.574e-17       & 1.623e-16       & 1.383e-16       & 1.521e-15 \\
    18 & 3.149 & (1, 3+1/8)  & 5.707e-16       & 2.357e-17       & 1.371e-15       & \bad 1.438e-02  & \bad 2.638e-04  & 5.981e-15 \\
    19 & 3.149 & (-1, 3+1/8) & 3.890e-16       & 3.388e-17       & \bad 2.615e-03  & 2.466e-15       & 2.766e-17       & 2.468e-15 \\
    20 & 3.149 & (3, 3+1/8)  & 3.232e-17       & 3.873e-17       & 1.050e-16       & 5.005e-16       & 3.959e-16       & \bad 3.337e-02 \\
    21 & 3.149 & (-3, 3+1/8) & 1.043e-16       & 2.178e-17       & 2.989e-15       & 2.642e-15       & 5.205e-16       & 6.698e-15 \\
    22 & 3.277 & (3, 3+1/8)  & 4.345e-16       & 1.803e-16       & 7.954e-16       & 1.264e-15       & 1.397e-14       & \bad 7.796e-01 \\
    23 & 3.277 & (-3, 3+1/8) & 3.241e-16       & 3.454e-17       & 5.567e-16       & 6.517e-16       & 2.187e-16       & 1.612e-13 \\
    24 & 4.000 & (0, 4)      & 1.099e-16       & \bad 7.547e-04  & 3.697e-17       & 5.693e-17       & 5.130e-17       & 3.125e-16 \\
    \bottomrule
  \end{tabular}
  \caption{\M{\phi_\beta}}
  \label{tab:ising_l2}
\end{table}

\begin{table}[htb]
  \centering\small
  \def\M#1{$\mel{\phi_\alpha}{\bar{L}_{+2}}{#1}$}
  \begin{tabular}{*{9}{c}}
    \toprule
    $\ket{\phi_\alpha}$ & $\Delta_\alpha$ & $(s_\alpha, \Delta^{\text{exact}}_\alpha)$ & \M{12} & \M{15} & \M{19} & \M{21} & \M{22} & \M{23} \\
    \midrule
    1  & 0.000 & (0, 0)      & 5.467e-15       & \bad 4.795e-03  & 1.856e-16       & 1.520e-16       & 5.713e-16      & 1.245e-16 \\
    2  & 0.123 & (0, 1/8)    & \good 9.867e-01 & 4.046e-15       & 2.586e-16       & 5.058e-16       & 9.216e-16      & 8.715e-16 \\
    3  & 0.990 & (0, 1)      & 3.940e-15       & \good 9.955e-01 & 1.994e-14       & 1.384e-14       & 1.628e-14      & 1.349e-15 \\
    4  & 1.119 & (1, 1+1/8)  & 6.594e-16       & 2.919e-15       & \good 9.841e-01 & 4.570e-13       & 1.000e-14      & 4.304e-13 \\
    5  & 1.119 & (-1, 1+1/8) & 6.964e-16       & 2.776e-15       & 3.919e-13       & \good 9.842e-01 & 2.353e-12      & \good 9.962e-01 \\
    6  & 2.000 & (1, 2)      & 2.966e-17       & 2.019e-16       & 3.288e-15       & 5.373e-16       & 2.381e-15      & 1.743e-16 \\
    7  & 2.000 & (-1, 2)     & 6.025e-17       & 3.039e-16       & 1.670e-16       & 4.959e-15       & 5.919e-16      & 1.318e-15 \\
    8  & 2.000 & (2, 2)      & 7.485e-17       & 2.251e-16       & 2.593e-16       & 2.083e-16       & 4.436e-16      & 2.246e-16 \\
    9  & 2.000 & (-2, 2)     & 7.495e-17       & 6.037e-16       & 3.122e-16       & 3.257e-16       & 1.903e-15      & 3.502e-16 \\
    10 & 2.114 & (0, 2+1/8)  & \bad 8.935e-04  & 9.438e-16       & 3.131e-16       & 3.338e-16       & 7.598e-16      & 2.725e-16 \\
    11 & 2.154 & (2, 2+1/8)  & 6.331e-16       & 9.592e-17       & 2.916e-16       & 1.403e-16       & 4.221e-16      & 2.540e-16 \\
    12 & 2.154 & (-2, 2+1/8) & 7.313e-16       & 1.787e-16       & 3.496e-16       & 4.773e-16       & 2.210e-15      & 4.931e-16 \\
    13 & 3.010 & (0, 3)      & 1.460e-15       & \bad 1.158e-03  & 6.726e-17       & 5.694e-17       & 1.475e-15      & 8.429e-17 \\
    14 & 3.072 & (2, 3)      & 3.628e-17       & 2.232e-16       & 2.778e-17       & 1.042e-16       & 1.397e-15      & 2.724e-17 \\
    15 & 3.072 & (-2, 3)     & 4.996e-17       & 1.423e-16       & 2.763e-17       & 1.681e-16       & 1.346e-15      & 4.588e-17 \\
    16 & 3.072 & (3, 3)      & 3.907e-17       & 5.139e-16       & 5.574e-17       & 1.623e-16       & 1.521e-15      & 1.383e-16 \\
    17 & 3.072 & (-3, 3)     & 3.601e-17       & 3.837e-16       & 1.870e-16       & 4.195e-16       & 1.606e-14      & 9.056e-17 \\
    18 & 3.149 & (1, 3+1/8)  & 3.890e-16       & 3.388e-17       & \bad 2.615e-03  & 2.466e-15       & 2.468e-15      & 2.766e-17 \\
    19 & 3.149 & (-1, 3+1/8) & 5.707e-16       & 2.357e-17       & 1.371e-15       & \bad 1.438e-02  & 5.981e-15      & \bad 2.638e-04 \\
    20 & 3.149 & (3, 3+1/8)  & 1.043e-16       & 2.178e-17       & 2.989e-15       & 2.642e-15       & 6.698e-15      & 5.205e-16 \\
    21 & 3.149 & (-3, 3+1/8) & 3.232e-17       & 3.873e-17       & 1.050e-16       & 5.005e-16       & \bad 3.337e-02 & 3.959e-16 \\
    22 & 3.277 & (3, 3+1/8)  & 3.241e-16       & 3.454e-17       & 5.567e-16       & 6.517e-16       & 1.612e-13      & 2.187e-16 \\
    23 & 3.277 & (-3, 3+1/8) & 4.345e-16       & 1.803e-16       & 7.954e-16       & 1.264e-15       & \bad 7.796e-01 & 1.397e-14 \\
    24 & 4.000 & (0, 4)      & 1.099e-16       & 7.547e-04       & 3.697e-17       & 5.693e-17       & 3.125e-16      & 5.130e-17 \\
    \bottomrule
  \end{tabular}
  \caption{\M{\phi_\beta}}
  \label{tab:ising_lbar2}
\end{table}

